Decentral and Incentivized Federated Learning Frameworks: A Systematic Literature Review

The advent of Federated Learning (FL) has ignited a new paradigm for parallel and confidential decentralized Machine Learning (ML) with the potential of utilizing the computational power of a vast number of IoT, mobile and edge devices without data leaving the respective device, ensuring privacy by design. Yet, in order to scale this new paradigm beyond small groups of already entrusted entities towards mass adoption, the Federated Learning Framework (FLF) has to become (i) truly decentralized and (ii) participants have to be incentivized. This is the first systematic literature review analyzing holistic FLFs in the domain of both, decentralized and incentivized federated learning. 422 publications were retrieved, by querying 12 major scientific databases. Finally, 40 articles remained after a systematic review and filtering process for in-depth examination. Although having massive potential to direct the future of a more distributed and secure AI, none of the analyzed FLF is production-ready. The approaches vary heavily in terms of use-cases, system design, solved issues and thoroughness. We are the first to provide a systematic approach to classify and quantify differences between FLF, exposing limitations of current works and derive future directions for research in this novel domain.

==> 40_methods.tex <==
\section{Method of Literature Review}
\label{sec:method}
The goal of the following systematic literature review is the identification of decentralized collaborative learning solutions where participation is rewarded. The aim of this study is not only to summarize all major publications, but also to extend the research by having a guideline for current and future practitioners.

Relevant publications are retrieved, filtered, and selected by a methodical procedure. The procedure is inspired by the Preferred Reporting Items for Systematic Reviews and Meta-Analyses (PRISMA) methodology~\cite{moher2015preferred}. PRISMA helps authors to improve the reporting of reviews. Within this work, the PRISMA methodology is augmented with the guide for information systems proposed by Okoli~\etal and Kitchenham~\etal~\cite{okoli2010guide, kitchenham2004procedures}. The guidelines are a structured approach to conduct a systematic literature review. They consist of five core steps: \one defining research questions, \two searching for literature, \three screening, \four reviewing, \five selecting and documenting relevant publication and extracting relevant information. The corresponding flow diagram of the conducted SLR is illustrated in \figurename~\ref{fig:tikz:prisma-diagram}.

\subsection{Research Questions}

The review and selection of relevant literature is conducted for extracting, preparing, and summarizing relevant information for future researchers.
The scope of relevant information is described and limited by five corresponding research questions.

\begin{enumerate}%[\setlabelwidth{RQ1}]
    % \item[RQ1] Applications: what are the applications and solved problems of decentral and incentivized FL frameworks within the scientific literature?
    \item[RQ1] Overview: \one What are possible applications of FLF? \two What problems were solved? \three Across which dimensions are the FLF papers heterogeneous?
    
    %\item[RQ2] Blockchain features: (i) How is blockchain applied in terms of computation, storage and type of framework to facilitate decentralization? and (ii) Is the framework scalable? 
    \item[RQ2] Blockchain: \one What is the underlying blockchain architecture? \two How is blockchain applied within the FLF and what operations are performed? \three Is scalability considered? 

    \item[RQ3] Incentive mechanism: \one How are incentive mechanisms analyzed? \two How are the contributions of workers measured?
    
    \item[RQ4] Federated learning: \one Is the performance of the framework reported? \two How comprehensive are the experiments? \three Are non-IID scenarios simulated? \four Are additional privacy methods applied? \five Is the framework robust against malicious participants?
    
    %\item[RQ5] Limitations: (i) what are major limitations and research gaps of contemporary works? and (ii) what are future directions to enable decentral and incentivized collaborative learning for mass adoption?
    %\item[RQ5] Summary and future work: (i) what are lessons learned from review? and (ii) what are potential future research directions?
    \item[RQ5] Summary: What are the lessons learned from the review?
\end{enumerate}



 \subsection{Search Process}
We conduct a well-defined search process of relevant publications to allow for reproducibility. The main keywords of interest are ``Federated Learning'', ``Blockchain'', and ``Game Theory''. Due to the existence of synonyms (e.g., ``Collaborative Learning'' instead of ``Federated Learning'') and abbreviations (e.g., ``DLT'' instead of ``Blockchain'') the search term is extended by taking these variations into account. The final case-insensitive search term is the following:
\begin{hyphenrules}{nohyphenation}

\begin{highlightBox}[Search Term]
  %\texttt{("Federated Learning" OR "Federated Artificial Intelligence" OR "Collaborative Learning") AND ("Blockchain" OR "Distributed Ledger" or "DLT") AND ("Mechanism Design" OR "Incentive" OR "Reward" OR "Game Theory" OR "game-theoretical" OR "Economics")}
  \texttt{(``Federated Learning'' OR ``Federated Artificial Intelligence'' OR ``Collaborative Learning'') AND (``Blockchain'' OR ``Distributed Ledger'' OR ``DLT'') AND (``Mechanism Design'' OR ``Incentive'' OR ``Reward'' OR ``Game Theory'' OR ``game-theoretical'' OR ``Economics'')}
\end{highlightBox}

\end{hyphenrules}

We selected 12 of the major computer science publication databases. The search was conducted on November 21, 2021. All search results retrieved at that date were taken as input for further manual inspection. The current results of the query can be obtained by following the hyperlink after each database entry below:
\begin{itemize}
\item IEEE Xplore Digital Library \href{https://ieeexplore.ieee.org/search/searchresult.jsp?newsearch=true&queryText=(%22Federated%20Learning%22%20OR%20%22Federated%20Artificial%20Intelligence%22)%20AND%20(%22Blockchain%22%20OR%20%22Distributed%20Ledger%20Technology%22%20OR%20%22DLT%22)%20AND%20(%22Mechanism%20Design%22%20OR%20%22Incentive%22%20OR%20%22Reward%22%20OR%20%22Game%20Theory%22%20OR%20%22game-theoretical%22%20OR%20%22Economics%22)}{(URL)}

\item SpringerLink Database
\href{https://link.springer.com/search?query=%28%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22%29+AND+%28%22Blockchain%22+OR+%22Distributed+Ledger+Technology%22+OR+%22DLT%22%29+AND+%28%22Mechanism+Design%22+OR+%22Incentive%22+OR+%22Reward%22+OR+%22Game+Theory%22+OR+%22game-theoretical%22+OR+%22Economics%22%29}{(URL)}

\item ACM Digital Library
\href{https://dl.acm.org/action/doSearch?AllField=(%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22)+AND+(%22Blockchain%22+OR+%22Distributed+Ledger+Technology%22+OR+%22DLT%22)+AND+(%22Mechanism+Design%22+OR+%22Incentive%22+OR+%22Reward%22+OR+%22Game+Theory%22+OR+%22game-theoretical%22+OR+%22Economics%22)}{(URL)}

\item ScienceDirect Database
\href{https://www.sciencedirect.com/search?qs=%28%22Federated%20Learning%22%29%20AND%20%28%22Blockchain%22%20OR%20%22Distributed%20Ledger%20Technology%22%29%20AND%20%28%22Mechanism%20Design%22%20OR%20%22Incentive%22%20OR%20%22Reward%22%20OR%20%22Game%20Theory%22%20OR%20%22game-theoretical%22%20OR%20%22Economics%22%29}{(URL)}


\item MDPI\footnote{As MDPI does not allow for nested search terms, we tried possible keyword combinations such as ``Federated Learning'' AND ``Blockchain'' AND ``Mechanism Design'' \href{https://www.mdpi.com/search?advanced=(@(all)%22Federated%20Learning%22@(all)Blockchain@(all)%22Mechanism%20Design%22)}{(URL)}}

\item Emerald insight
\href{https://www.emerald.com/insight/search?q=%28%22Federated%20Learning%22%20OR%20%22Federated%20Artificial%20Intelligence%22%20OR%20%22Collaborative%20Learning%22%29%20AND%20%28%22Blockchain%22%20OR%20%22Distributed%20Ledger%22%20OR%20%22DLT%22%29%20AND%20%28%22Mechanism%20Design%22%20OR%20%22Incentive%22%20OR%20%22Reward%22%20OR%20%22Game%20Theory%22%20OR%20%22game-theoretical%22%20OR%20%22Economics%22%29&showAll=true&ipp=50&p=1}{(URL)}

\item Talor \& Francis \href{https://www.tandfonline.com/action/doSearch?AllField=%28%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22+OR+%22Collaborative+Learning%22%29+AND+%28%22Blockchain%22+OR+%22Distributed+Ledger%22+OR+%22DLT%22%29+AND+%28%22Mechanism+Design%22+OR+%22Incentive%22+OR+%22Reward%22+OR+%22Game+Theory%22+OR+%22game-theoretical%22+OR+%22Economics%22%29}{URL}

\item Hindawi
\href{https://hindawi.com/search/all/(%22Federated%20Learning%22%20OR%20%22Federated%20Artificial%20Intelligence%22%20OR%20%22Collaborative%20Learning%22)%20AND%20(%22Blockchain%22%20OR%20%22Distributed%20Ledger%22%20OR%20%22DLT%22)%20AND%20(%22Mechanism%20Design%22%20OR%20%22Incentive%22%20OR%20%22Reward%22%20OR%20%22Game%20Theory%22%20OR%20%22game%20theoretical%22%20OR%20%22Economics%22)/page/1}{(URL)}

\item SAGE 
\href{https://journals.sagepub.com/action/doSearch?filterOption=allJournal&AllField=%28%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22+OR+%22Collaborative+Learning%22%29+AND+%28%22Blockchain%22+OR+%22Distributed+Ledger%22+OR+%22DLT%22%29+AND+%28%22Mechanism+Design%22+OR+%22Incentive%22+OR+%22Reward%22+OR+%22Game+Theory%22+OR+%22game-theoretical%22+OR+%22Economics%22%29}{(URL)}

\item Inderscience online 
\href{https://www.inderscienceonline.com/action/doSearch?AllField=%28%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22%29+AND+%28%22Blockchain%22+OR+%22Distributed+Ledger+Technology%22+OR+%22DLT%22%29+AND+%28%22Mechanism+Design%22+OR+%22Incentive%22+OR+%22Reward%22+OR+%22Game+Theory%22+OR+%22game-theoretical%22+OR+%22Economics%22%29}{(URL)}

\item Wiley
\href{https://www.wiley.com/en-us/content-search?cq=%28%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22+OR+%22Collaborative+Learning%22%29+and+blockchain&pq=%28%22Federated+Learning%22+OR+%22Federated+Artificial+Intelligence%22+OR+%22Collaborative+Learning%22%29+and+%28%22Blockchain%22+OR+%22Distributed+Ledger%22+OR+%22DLT%22%29&pq=%28%22Blockchain%22+OR+%22Distributed+Ledger%22+OR+%22DLT%22%29+and+%28%22Mechanism+Design%22+OR+%22Incentive%22+OR+%22Reward%22+OR+%22Game+Theory%22+OR+%22game-theoretical%22+OR+%22Economics%22%29}{(URL)}
\end{itemize}

After applying the search term, we found \rawresults publications overall. In addition to this search, the references were screened and \resultsreference more eligible paper was found and included for analysis.

Each publication that we retrieved based on our search was exported or enriched by 
\one document title,
\two abstract,
\three author names,
\four publication year, and
\five Digital Object Identifier (DOI).

% https://tex.stackexchange.com/a/51761
\begin{figure}[t]
    \centering
    %\includestandalone[width=0.46\textwidth]{PRISMA_grafik_org.tex}
    \resizebox{\columnwidth}{!}{%
        \input{PRISMA_grafik_org}
    }
    \caption{PRISMA diagram.}
    \label{fig:tikz:prisma-diagram}
\end{figure}
%\Figure[!t]()[width=0.46\textwidth]{PRISMA_grafik_org.tex}
%{PRISMA diagram\label{fig:tikz:prisma-diagram}}

\subsection{Selection Process} 
The eligibility of the literature corpus that we gathered based on the string was evaluated independently by three researchers. 
%For this, all studies were aggregated in three separate spreadsheets, one per researcher. Then, 
Duplicates were removed and several iterations of manual verification were performed.
First, we present the criteria that we applied to include (or exclude) an article for further consideration.
Then, we discuss our manual eligibility check.

\subsubsection{Inclusion and exclusion criteria}\label{sec:inclusion}

The following three criteria must be fulfilled by an article in order for it to be included for further analysis:
\begin{enumerate}
    \item The article must have a direct relation to all of the three search terms \one Federated Learning \& \two  Blockchain \& \three Mechanism Design or their respective synonyms. 
    
    \item The article must be of full length to explain proposed architectures and concepts in depth. 
    
    \item The article must be written in English.
\end{enumerate}

%The following exclusion criteria prevent not relevant articles from passing the filter process.
If the article matched one of the following three criteria, it was excluded from further analysis:
\begin{enumerate}
    
    \item Articles which do not discuss collaborative learning in the context of both decentralization and incentives. This also covered articles which discuss only two of the three major terms or consider the search terms in a different context.
    
    \item Short papers such as poster abstracts because they do not cover enough information to provide a sufficient level of understanding.
    
    \item Vague articles which only give an brief overview about the topics, e.g., superficial descriptive articles were excluded.
\end{enumerate}


\subsubsection{Manual eligibility check}
The following manual eligibility checks were performed by the authors:

\begin{enumerate}
    \item Removal of faulty or correction of incorrect lines in the aggregation file that includes all search results.
    \item Reading the titles and abstracts of the articles. Each article was marked as follows based on our inclusion criteria, see Section~ \ref{sec:inclusion}: 
      \begin{enumerate}
        \item Include, if the article should be included.
        \item Exclude, if the article should be excluded.
        \item Not sure, if the article should be re-checked against the defined criteria and briefly discussed.
      \end{enumerate}
    
    \item The authors compared and discussed their assessments. Disagreements were highlighted and handled as follows: The article was re-checked against the defined criteria and briefly discussed. Sometimes one researcher noticeably misinterpreted the research focus of an article. In that case the article was excluded. In all other cases the article was included.
    \item Reading parts of or the complete full text in order to get a deeper insight into the research. Then, the article was again voted for inclusion or exclusion.
    \item The authors compared and discussed their respective selected papers. The same decision levels as described in 2) were used for the comparison.
    \item The authors read all eligible papers independently and extracted all necessary information.
    \item Discussion of findings and information exchange.
\end{enumerate}

If the decision on the eligibility of a paper was not clear after further consideration, the authors decided on including the respective article. All included articles were read and relevant information was extracted.

\subsection{Screening Process}
In order to cover as much structured information as possible, the analysis of the papers was guided by predefined categories regarding the FL framework (\tablename~\ref{table:FL}), blockchain features (\tablename~\ref{table:blockchain}), incentive mechanism features (\tablename~\ref{table:incentive_mechanism}) and the experiment analysis (\tablename~\ref{table:experiments}). After conducting all steps described above, a total of \finalresults articles remain that match the initially defined scope of this structured literature review and are further processed to answer the research questions.

==> 51_results_summary.tex <==
\subsection{Summary}
\label{sec:summary}
Witt \etal established a generic fully decentralized FL framework utilizing federated knowledge distillation on 1-bit compressed label predictions of a public dataset to train the federation \cite{LW1_witt2021rewardbased}. The adjustment of the peer truth serum mechanism for the FL case allowed for informed-truthful signal elicitation as well as a fair and lightweight profit allocation among participants through a smart contract. 

Weng \etal  introduced a distributed, secure and fair deep learning framework named DeepChain \cite{LW2_Weng2021}. The introduced application-specific blockchain system in detail and implemented a prototype. Their incentive mechanism is novel yet lacks theoretical analysis.

Kumar \etal proposed a decentralized training framework on Ethereum, applying elastic weight consolidation against catastrophic forgetting and differential privacy as well as homomorphic encryption to enhance privacy. Yet, the framework lacks detail \cite{LW3_Kumar2020}.

Zhang \etal proposed a blockchain-based federated learning system for failure detection in IIoT \cite{LW4_FL_IIoT}. They apply centroid distance weighted federated averaging to get better results in non-iid environments and applied a smart contract based incentive mechanism. The experiments are conducted on real life data of AC machines.

Zhao \etal introduced a privacy preserving blockchain based federated learning for smart home systems. Data from IoT devices get collected with a smart phone before it gets sent to a mobile-edge computing server. They developed a novel normalization technique and reward participation based on the euclidean distance of the gradients.



%Bao \etal proposed a blockchain system dedicated to federated learning called FLchain \cite{Bao2019FLChain}. The proposed system takes an on-chain strategy, storing all the information in the blockchain and aggregating model updates in the smart contract. Anyone can report misbehaviors to the smart contract, and FLchain checks its claim and penalizes dishonest workers if necessary.
Bao \etal propose a deposit- and peer-evaluation based FL framework called FLchain with privacy protection through masked gradients \cite{Bao2019FLChain}. The proposed system takes an on-chain strategy, storing all the information in the blockchain and aggregating model updates in the smart contract. Anyone can report misbehaviors to the smart contract, and FLchain checks its claim and penalizes dishonest workers if necessary.The participants gain profit by offering their model on a public marketplace.

Martinez \etal proposed an incentive-aware federated learning platform with blockchain \cite{Martinez2019}. They store gradients off-chain while its hashes are stored in the blockchain to save blockchain size. Reward is determined by data size used for training and given only when a model is improved. However, the data size and quality improved via training are based on ``self-report,'' meaning this method must rely on users' reports. They have implemented smart contracts using Hyperledger Fabric, while stating that they will reimplement it with the EOS blockchain.

Toyoda \etal proposed a competition-based approach to determine the winners of prizes by voting \cite{Toyoda2019, Toyoda2020}. The incentive mechanism is analyzed using contest theory under different risk assumptions (i.e. risk averse or risk neutral).



%\cite{Chai2021}MH1
Chai \etal propose a FL framework with two aggregation layers for the IoV domain \cite{MH1_Chai2021}. The hierarchical structure promotes scalability. The incentive mechanism is designed as multi-player non-cooperative Stackelberg game. Blockchain technology is used to securely share the model weights between the hierarchy levels and to conduct the payment of rewards.

%\cite{Kang2019}MH2
Kang \etal develop a multi-weight subjective logic for computing the participants' reputation scores which are key to their FL framework \cite{MH2_Kang2019}. For that, specific attack detection schemes are utilized for iid and non-iid scenarios (RONI, Fool's-Gold). Furthermore, the authors compare FL approaches that are based on Stackelberg games and contract theory.

%\cite{Bao2019FLChain}MH3
%Bao \etal propose a deposit- and peer-evaluation based FL framework with privacy protection through masked gradients \cite{Bao2019FLChain}. The participants gain profit by offering their model on a public marketplace.

%\cite{Ma2021}MH4
Ma \etal develop a method for secure contribution measurement \cite{MH4_Ma2021}. Since the native way of computing Shapely value does not work on masked updates, Shapley values for groups of clients are determined. Furthermore, they integrate their method in a dezentralized FL framework and demonstrate the method's feasibility.

%\cite{Lei2021}MH5
Feng \etal employ a framework based on two BC layers \cite{MH5_Lei2021}. They ensure scalability through BC sharding and device-to-device (D2D) communication. The design of contracts despite incomplete information is realized by information prediction through deep neural networks.

%\cite{Kansra2022}MH6
\todo{@Kentaroh: This one maybe interesting for IM paragraph/table, since they somehow incoporate data augmentation:} Kansra \etal integrate data augmentation into their framework to increase model accuracy \cite{MH6_Kansra2022}. At the same time, this additional task is the basis for their incentive mechanism. The participants have to complete two tasks: local model training and augmentation of their data. The augmented data sets are uploaded to the chain, pooled, and relayed to all edge nodes. Clients with better model updates compared to the competing nodes have to perform less data augmentation in the next training round and thereby save computation costs.

%\cite{Mugunthan2022}MH7
Mungunthan \etal propose a privacy-preserving and trust-less framework including a contribution scoring procedure that allows contribution measurement and thereby effective incentive design and prevention of malicious attacks \cite{MH7_Mugunthan2022}.

%\cite{Fadaeddini2019}MH8
Fadaeddini \etal employs a Stellar-based framework \cite{MH8_Fadaeddini2019}. The incentive mechanism requires customers to pay higher participation fees if they have engaged in malicious behavior previously. The payment is conducted using an internal currency, malicious behavior is detected by validators who test the submitted models on a not further specified test set.

%\cite{He2021}MH9
\todo{@Kentaroh: This one maybe interesting for IM paragraph/table, see group chat:} He \etal propose a flexible framework for horizontal and vertical FL \cite{MH9_He2021}. An incentive mechanism is designed that independently rewards maintaining the blockchain, participating in FL, and contributing high-quality data to FL. For the latter, each participant's contribution is determined in multiple steps, including (1.) a pre-filtering based on the Euclidean distance between the model update and the mean of all model updates, and (2.) the computation of the Shapley value.

%MH10
\todo{@Leon: This one maybe interesting for blockchain paragraph/table, since own Consensus Mechanism:} Qu \etal introduce decentralized, federated learning to offloading decision making with deep neural networks \cite{MH10_Qu2021}. They develop a consensus mechanism that is more efficient than PoW and in addition prevents poisoning attacks by incorporating the "average reward value" of the local offloading decision model. 

%MH11
\todo{@Leon: This one maybe interesting for blockchain paragraph/table, since use of both private and public:} Desai \etal develop a hybrid blockchain-based FL framework that combines a private and a public blockchain to prevent backdoor attacks\cite{MH11_Desai2021}. By introducing accountability and a penalty mechanism, malicious agents can be detected and punished a posteriori once a backdoor is identified. The two employed blockchain types compensate each others weaknesses: The aggregation calculations are conducted on the lower-latency private blockchain, whereas the public blockchain is used for payment processing and ensures accountability through public parameter storage. 

%MH12
Zhu \etal incorporate secure multi-party aggregation into their framework for privacy-preserving federated learning \cite{MH12_Zhu2021}. Furthermore, they evaluate the performance and privacy-preserving property of their architecture in experiments with up to 900 participants.

%MH13
Li \etal propose a federated learning framework for crowd computing \cite{MH13_Li2020}. In each FL round, only the best few model updates are considered for aggregation. To identify these, a scoring evaluation mechanism based on model accuracy, training data size, and reputation is developed. Furthermore, Elgamal-based encryption promotes data privacy.

%MH14
Rathore \etal develop and test a blockchain-based FLF for the IoT domain, where the computationally intense model aggregation and mining tasks are performed by edge servers, whereas the IoT devices only participate in local model training and do not serve as blockchain miners or aggregators \cite{MH14_Rathore2019}.




Hu \etal proposed a blockchain-enabled federated learning for mobile crowdsensing. Sensing data are collected by users and sent to edge servers for training. The edge servers collaboratively train a model with FL. The authors formulated utilities of users and edge servers, which considers payoffs and the cost of sensing and privacy leakage, and derived their optimal strategies by maximizing the utilities. A consortium blockchain is used to enable FL among edge servers. \todo{insert citation here please}

Wang \etal proposed a blockchain-based FL architecture for UAVs to securely exchange local model updates and verify contributions without a central server. They also propose a privacy-preserving algorithm with differential privacy to protect UAVs' privacy of updated local models. A two-tier reinforcement learning-based incentive mechanism is designed to promote UAVs' high-quality model sharing when explicit knowledge of network parameters are not available in practice.\todo{insert citation here please}

ur Rehman \etal proposed a three-tier fine-grained FL architecture. The architecture enables to perform FL on-device, on-edge, and on-cloud. The public Ethereum blockchain is used to manage users' reputation scores.\todo{insert citation here please}

Qu \etal propsoed a new consensus algorithm for blockchain called proof of federated learning (PoFL). Two approaches, namely a reversed game-based trading mechanism and privacy-preserving model verification, are proposed to enable model performance verification without privacy concerns.\todo{insert citation here please}



Zhang \etal introduced Refiner, an incentive-driven FL system on blockchain to enable massive engagement in FL \cite{LW10_refiner}. The system comprises of a registry contract and a task contract, where requesters start a round, Workers train the models and validators audit the workers contribution.

Jiang and Wu introduced a reward-response Stackelberg game in blockchain-powered FL \cite{LW11_RewardResponseGame}. They analyzed the game-theoretic properties for both, size-based and accuracy-based contributions of workers while taking client-sided upload times into consideration.


Rahmadika \etal introduced a novel privacy-aware collaborative learning framework for the decentralized cross-silo FL \cite{LW12_Rahmadika2021_unlinkable}. Implemented using the Ethereum Virtual Machine (EVM), their framework allows for unlinkable and untraceable transactions utilizing ring-signatures. The paper conducted a thorough Ethereum-gas analysis of their implementation. A reward system is mentioned yet not specified.

Habib ur Rehman \etal introduced a reputation aware framework for fine-grained FL, where reputation scores are stored on the blockchain \cite{TowardsReputationINFOCOMM}. The framework is introduced only a generic concept, the reputation calculation is not specified in detail and the framework lacks validation through experiments.

.

==> 60_discussion.tex <==
% \section{Challenges in Comparing FLF}

% \paragraph{RQ 5} \textit{What  are  the major challenges in comparing FLF? What do practitioners need take into consideration?}


\section{Discussion}
\label{sec:discussion}


\paragraph{RQ 5} \textit{What  are  major  limitations  and  research  gaps  of contemporary  works?  What  are  future  directions to  enable  decentral  and  incentivized  collaborative learning for mass adoption?}
% Mathis introduction
% A powerful comparison framework would noticeably serve the advancement of the technology, as it would result in a clearer solution approach accounting and in the effectiveness of the proposed approaches being comparable. The comparison framework should specify clearly defined building blocks and characteristics of FLFs. This categorization should be as specific as possible, but as generic as necessary to ensure applicability to all domains and to not confine creativity in the FLF design process.   

The preceding analysis of the papers in terms of the FL framework, the use of blockchain, the design of an incentive mechanism, and the conduct of experiments has yielded four findings. \one The existing research is characterized by significant \textbf{heterogeneity} in various dimensions. Through our definition of 26 characteristics, we attempt to bring structure to this heterogeneity and better expose the differences and similarities among existing frameworks. \two In some of the categories, competing solutions exist with different tradeoffs. When designing a framework, a choice must be made here, which we seek to support by briefly outlining these tradeoffs below. \three Some recurring approach-related and methodological shortcomings exist, the avoidance of which would further improve future research. \four Beyond better understanding the aforementioned trade-offs, there are a number of unresolved issues waiting to be addressed by future research.

% The current research ranges from mere ideas to proof of concepts. None of the proposed frameworks are currently used for real-world applications. Based on our research, we propose four actions that are essential to exploit the benefits of decentralized, incentivized FL frameworks and to establish them in industry. There is a need to \one pinpoint and avoid repeatedly occurring shortcomings of the frameworks, \two develop a comprehensive comparison framework, \three resolve the remaining technological challenges, and \four explore new ideas in the field of decentralized, incentivized FL. In this section we elaborate on these four actions.


% In order to apply incentivized and decentralized FLF in production, the contemporary state-of-the-art research has to be taken into comparison with respect to its use-case, properties and scalability.\todo{@Kentaroh you said this logic is not correct?}
\subsection{Heterogeneity of Existing Work}
This work identified heterogeneity of FLF in the four dimensions, namely \one application, \two overall design, \three special focus on open issues and \four details and thoroughness. In order to overcome this challenge, we categorize the FLF characteristics into general characteristics, blockchain-related characteristics, incentive mechanism-related characteristics, and experiment-related characteristics (Table~\ref{tab:columns_definition})


%In particular, we developed a detailed comparison framework with respect to the general use-case and key contributions, the use of blockchain technology, the incentive mechanism and the conducted experiments to enhance adaptation through transparency. 

% The a heterogeneity in the four dimensions, namely \one application, \two overall design, \three special focus on open issues and \four details and thoroughness challenged the pursuit of fair comparison. The introduced comparison framework of this work is to give 
% @Leon Include!
% The systematic we used to categorize the proposed FLFs provides a good starting point for such a comparison framework. Our framework is applicable domain-independently, and at the same time detailed and comprehensive. 


\textbf{Application} Although the majority of analyzed works offered application independent frameworks (classified as generic in table~\ref{table:FL}) other FLF are applied across IoT, IIoT, IoV and Finance. The heterogeneity of the required properties across those domains lead to vast differences in the design choices of function, operations and storage of blockchain, contribution measurement and privacy requirements. 

\textbf{Variety of possible design choices} In addition to the domain specific influence on the design choice, design choices about the FL algorithms, communication protocol, applications of blockchain within the ecosystem, blockchain technology (existing or novel), storage and operation on blockchain, security trade-offs, mechanism design, contribution measurement, etc. add to the complexity and overall variety of such systems. For example, some works apply blockchain at its outer complementary layer \cite{} while blockchain being the core infrastructure to coordinate, store, aggregate and payment in other FLFs \cite{LW1_witt2021rewardbased, LW10_refiner}. Furthermore, some works developed application specific blockchain systems, while others try to embed an FLF on top of existing blockchain frameworks such as Ethereum for cheaper and pragmatic deployment. Our survey exposes a similar variety in the choice of the contribution measurement: The spectrum reaches from computationally light-weight correlation of answers on a public dataset \cite{LW1_witt2021rewardbased} as a  proxy for contribution as apposed to the Shapley value, a measurement with strong theoretical properties at the cost of massive computational overhead \cite{LW9_FedCoin,MH9_He2021}. 
% Wonanders

\textbf{Special Focus} The aforementioned complexity as well as its novelty result in many open issues across a broad spectrum. Many works therefore focus on solving specific issues such as enhanced privacy \cite{LW2_Weng2021, LW8_Privacy_IoV,LW12_Rahmadika2021_unlinkable, MH8_Fadaeddini2019}, a novel blockchain systems \cite{LW4_FL_IIoT,LW9_FedCoin}, bandwidth reduction \cite{}, novel contribution measurements \cite{LW1_witt2021rewardbased, LW9_FedCoin, MH10_Qu2021} or game theory (e.g., \cite{MH2_Kang2019, LW11_RewardResponseGame}), as the major contribution which further complicates a comparison of the holistically of FLF.\todo{@Kentaroh: Please insert some examples from your papers whith a very specialized focus on a certain issue}

\textbf{Thoroughness} The analyzed papers also vary heavily in provided detail and thoroughness, ranging from first concepts, lacking details in terms of important specifications such as performance, specific function, operation and storage on blockchain, contribution measurement, robustness, experiments and privacy to theoretically detailed and experimentally tested solutions. None of the analyzed papers are production-ready.

% Deleted this because we cant blame anyone for picking some descriptive name instead of another, and because the slightly ambiguous use of "secure aggregation" can be quickly understood by reading one or two papers. 
%\textbf{Inconsistent Nomenclature}
%Moreover, inconsistent nomenclature across the publications makes it difficult to compare the frameworks. This is particularly noticeable in the nomenclature of the actors and the characterization of the privacy mechanisms used.\todo{@Mathis can you give some explicit examples+citations here?} 
These varieties emphasize the additional layer of complexity when quantifying differences.


% The scientific literature should provide sufficient information about the use of blockchain and the incentive mechanism in order to be comparable.

\subsection{Design choices under trade-offs}
%Across the analysed papers we identify a series of shortcomings. We further clustered these into Scalability, Performance comparison, Lack of Specification, Assumptions, Mismatch between proposed system and experiments as well as Privacy protection. 

The following design choices in developing an FLF are characterized by particularly high-impact tradeoffs. 

\subsubsection{Blockchain: Decentralization vs Scalability}  yet particularly influential on the overall scalability. The scalability is determined by \one the function of blockchain in the FLF, \two operations performed onchain, \three blockchain framework and \four the amount of storage onchain. In particular, blockchain becomes a scalability bottleneck 
\begin{enumerate}
    \item if it is part of the operating core infrastructure of the FLF (e.g., \cite{LW1_witt2021rewardbased}) and not only a complementary outer layer technology (e.g., \cite{LW7_Zhang_Reputation})
    \item if heavy operations such as aggregation or reward calculation is performed on-chain \cite{LW9_FedCoin} 
    \item if the Blockchain framework is public and used outside the realm of the FLF or the consensus mechanism is based on resource-intense Proof of Work
    \item if heavy amount of information are stored on the blockchain such as model updates 
\end{enumerate}

Blockchain enables trust, immutability and decentralization for the operations and the information stored on it, yet come at the cost of low performance and limited scalability. 

\subsubsection{Contribution Measurement: Assumption vs Correctness}
Measuring workers' contribution is open research and vary heavily in the analyzed literature. Ranging from assuming full information, where the rewards are basically distributed based on the workers report of the amount of data or local accuracy towards report-correlations, reputation and Shapley Value. These metrices range from no calculation (full information case) to accuracy measures based on a test-set to heavy calculations such as Shapley-value. The Shapley value of cooperative game theory is a common method to measure the contribution of an agent in FL due to it's desired properties of efficiency, symmetry, linearity and null-player, yet come at the cost of heavy computational overhead, limiting the scalability of the framework. 
\todo{Kentaroh can you check this please?}
%The analyzed FLF offer several solutions ranging from data size as proxy under the (unrealistic) assumption of perfect information of the system over computationally cheap Correlation based predictions towards computational heavy measures such as Shapley value \cite{LW9_FedCoin,MH9_He2021}. The Shapley value calculates the marginal utility added per input feature, given all possible combinations. In this context $U(S) = U_m(A(S))$ represents the utility function where $A(\cdot)$ represents a learning algorithm that maps a dataset $S$ onto a model and $U_m(\cdot)$ is some measure of model performance, such as test accuracy. Retraining the model for each possible combination of participants requires an enormous computational overhead limiting the overall scalability of the system dramatically, even with improved algorithms for the Shapley value calculation in FL \cite{}. 

\subsubsection{Privacy Protection: Security vs. Accuracy/Overhead}
Despite FL being a data privacy preserving technology by design, research has shown that certain characteristics of the underlying training data sets can be inferred from the global model and that additional privacy preserving measures are recommended. Our review shows that two classes of security concerns are targeted by the publications: leakage of data set characteristics and disclosure of participant identities. Although a substantial number of papers (20 out of 40 publications) addresses one of these concerns, only a single paper adresses both~\cite{LW8_Privacy_IoV}. Moreover, especially preventing data set leakage through DP or MPC inflicts tradeoffs. Differential privacy comes with a trade-off between data security and model accuracy, and secure multi-party computing can establish data security according to high cryptographic standards, but requires more expensive computations and might thus not be applicable with a large number of participants~\cite{MH4_Ma2021}. On the contrary, Bonawitz~\etal~\cite{MH_SECURE_AGG} point out that some MPC algorithms have become more computationally efficient and can be applied with hundreds of users. 

\subsubsection{Complexity Trade-off} 
FLF specific blockchain systems claim to solve important shortcomings of existing blockchain frameworks, e.g., replacing the computational overhead of the Proof of Work systems with computational heavy tasks in FLF like model parameter \cite{KT08_Qu2021TPDS} or reputation verification \cite{LW7_Zhang_Reputation} or calculate the contribution measurement
\cite{LW9_FedCoin}. Other FLF specific blockchain systems utilize efficient AI hardware \cite{KT09_Zhang2021IJHPSA} or enhance the overall privacy for the FLF processes \cite{LW2_Weng2021} . Yet in the scientific literature widely ignored topic is the incurred deployment and maintenance cost of unproven novel blockchain systems in practice. Introducing a new, highly complex infrastructure unproven of practical introduces security risks and requires a large team of experts to run and maintain such a system in practice. Deployment on already existing blockchain frameworks may mitigate the additional complexity and risks.


\subsubsection{Assumptions: Realism vs Pragmatism} \todo{@Kenraroh}


%\begin{itemize}
    %\item Lack of consideration of scalability. Out of the 40 analyzed papers, only 6 mentioned the problem of scalability of the framework. Yet none of the solutions offer a quantifyable comparability.
    %\item No consideration of storage and computational effort on the blockchain as limiting factor for scalability
    %\item Inconsistent nomenclature is used (c.f., actors, privacy algorithms).
    %\item non-specific claims of blockchain application
    %\item Most experiments do not go beyond simple MNIST datsets. More complex datasts and ML tasks beyond classification are necessary to proof viability.
    %\item too simple benchmark data sets
    %\item Mismatch between proposed system and experiments (contradiction: \#clients vs. FL setting, BC implementation)
    %\item KT: Difference of Assumptions (Examples?!)
    %\item Performance not specified in terms of accuracy or loss. Ideally, the effectiveness of incentive mechanism and decentralization efforts are reflected in the FLF performance through a holistic experimental design.
    %\item different data sets
    %\item lack of detailed specification of infrastructure, blockchain details, contribution measurement
    %\item lack of non-iid consideration (in experiments) and its respective performance
    %\item dont test robustness to adversarial behavior (in experiments)
    %\item Privacy: Usually identity protection OR gradient masking, not both.
    %\item Deployment and maintenance cost of ASBS compared to existing and provem systems s.a. Ethereum not discussed
%\end{itemize}



\subsection{Common shortcomings}

Future researching efforts would be further improved by a stronger focus on the following recurring approach-related and methodological shortcomings that were observed in this systematic literature review. 

\subsubsection{Unrealistic Assumption}
Complete information: Measurement of \todo{@kentaroh}

\subsubsection{Limited Scalability consideration} One of the major factors of the applicability of a FLF is its ability to scale beyond small groups towards mass adoption. Out of the \finalresults papers, only 6 explicitly mentioned and considered scalability within the design of their respective FLF. 


\subsubsection{Lack of Specification}
As shown in Tables~\ref{table:FL}-\ref{table:experiments}, certain FLF properties are particularly prone to being specified only superficially. These include, in particular, the targeted FL setting, the exact implementation of the blockchain, the metrics of contribution measurements, and the FL algorithm used. To ensure the traceability and usability of the frameworks, careful specification should be made here. 

\subsubsection{Performance of the FLF} The overall objective of FL is to capitalize on untapped confidential data-silos to increase the performance of a global model to the mutual benefit of all participants. Yet, 11 out of 40 works did not consider the performance of the respective Framework. In order to have a meaningful performance measure, experiments on the FLF have to go beyond Classification (29 out of 32) of simple MNIST/FMNIST (20 out of 29 Classification tasks) towards a broader variety of different ML task such as NLP and user behavior analytics. In order to simulate a realistic environment, various levels of non-iid behavior and has to be taken into consideration into the performance measurement. Yet, out of 34 only 11 works have considered non-iid behaviour. 

% Furthermore, the effectiveness of incentive mechanism and decentralization efforts should ideally be reflected in the FLF performance through a holistic experimental design.

\subsubsection{Mismatch Between Proposed FLF and Experiments}
The experiments should demonstrate the feasibility of the framework in the best possible way. In addition to the aforementioned fact that very simple benchmark datasets are often used, the following mismatches stand out. First, the majority of publications (18 out of 33 papers with experiments) do not implement an actual blockchain in their experiments although proposed in their framework. There is a risk that scalability, cost and effort issues are underestimated. Furthermore, inconsistencies between the targeted FL setting (cross-silo, cross-device) and the number of clients in the experiments are observed. Especially, paper that propose cross-device frameworks tend to use or simulate an insufficient number of participating devices. Among the cross-device frameworks, only Kang~\etal~\cite{MH2_Kang2019} and Desai~\etal\cite{MH11_Desai2021} conduct experiments with 100 participants or more (\tablename~\ref{table:experiments}). 
%Finally, a series of frameworks claims the property of robustness against adversarial attacks, but does not simulate them in the experiments. Whenever attacks are simulated, different approaches are taken which are difficult to compare. 



\subsection{Future Research Suggestions}
Future research should not only focus on better understanding the aforementioned trade-offs (e.g., contribution measurement), but should also be concerned with solving the following open research gaps and exploring the following new ideas in the field. 

%Leons suggesions
1.) Scalability has to be explored in greater detail. 
2.) Trade-off between contribution measurement and the privacy of the user



%\subsubsection{Inexplainability of Workers' Behavior}
%We see that 12 out of 40 give theoretical analysis of the designed incentive mechanisms in some way. However, such analysis might not guarantee the robustness of the mechanisms. 
Even a theoretical analysis of the designed incentive mechanisms, as performed by 12 out of 40 papers, might not guarantee the robustness of the mechanisms. Specifically, as workers are humans, they may not follow their optimal strategies derived by analysis. For instance, not all the workers would take into account the cost of energy consumption when determining their strategies. Hence, it would be nice to take into account humans' behavioral bias into theoretical analysis. The prospect theory incorporates such bias into utility and probability calculation \cite{Kahneman1979, Tversky1992} and could be integrated with the FL incentive mechanism. This would result in more realistic workers' behavior as well as requesters' optimal reward allocation.

\textcolor{red}{Another open research question is the application of FL to more machine learning tasks beyond supervised learning~\cite{FedProx}. Especially in domains such as natural language processing or user behavior analytics, unsupervised learning tasks rely on more complex neural network architectures. These might require new or adapted model aggregation algorithms that might come with new implications on the incentive design and blockchain integration.}

Furthermore, we expect the application area of decentralized and incentivized FL to expand beyond the IoT and IoV domain, e.g., into the biomedical field. More generally, the technology is expected to become relevant to every domain where data is maintained separately but the data holders would benefit of joint ML model training. These novel use cases will bring further domain-specific challenges, e.g., with respect to data privacy requirements. 

\textcolor{red}{Li~\etal~\cite{FedProx} pointed out the issue of asynchronous communication. Currently, most frameworks assume a constant availability of the devices for participating in the FL task. Some frameworks are even designed to exclude participants from the entire FL process if they do not respond timely. However, more realistic scenarios have to be considered where the devices only pull tasks when their computational workload permits.}    


% später
% \section{Limitations of this work}
% This study is a systematic literature review, which naturally holds a number of limitations. As with the majority of studies, the design of the current study is subject to limitations and to a certain extend not fully objective. However, the authors tried to limit the subjectiveness by introducing an approach as structured as possible.

% \begin{itemize}
%     \item This study was limited by the search term and databases used. The study need to be replicated by using another similar search term or other databases to confirm the results. However, the 12 databases used in this review cover the majority of relevant publications.
%     \item Article selection and data analysis were done by three researchers. The decision made were limited by these researchers. %Having more researchers could have an impact on the results and strengthen the study.
%     \item The research articles resulting from the search term and databases are the basis for categorizing articles into different groups. The results extracted from the articles and the categories introduced are limited to articles found.
% \end{itemize}

% Summarized, the articles discussed in this systematic literature review provide an insight into the current research trend of this field and show the future research direction.

%\subsection{Limitations and future directions}\label{limitation}

%\subsubsection{Heterogeneity of frameworks}
%Application
%Overall Design - Where is blockchain used
%Special Focus on open issues
%Huge differences in details and theoretical analysis


%\begin{enumerate}
    %\item Lack of scalability consideration
    %\item mismatch between proposed system and experiments
    %\item no production ready system
    %\item storage as well as computational influence on scalability almost always ignored.

    %With this paper we tried to provide properties to ensure easy comparison
    %\item not a single FLF in production without real-life utility, spectrum from mere ideas to Proof of Concepts at best
    %\item KT: Difference of Assumptions (Examples?!)
    %\item KT: More realistic theory of the analysis

    %\item Blockchain aspects not compareable: Wide range from non-specific claim of blockchain application to a detailed implementation taking technical issues such as scalability, bandwidth, comparability into consideration
    %\item lack of comprehension: Most frameworks lack a detailed specification in all relevant areas, namely infrastructure, blockchain details, contribution measurement, validation through experiments, robustness against adversial behavior as well performance under several non-iid assumptions
    %\item Experiments: (1) "Ideally, the effectiveness of incentive mechanism and decentralization efforts are reflected in the FLF performance through a holistic experimental design."". (2) Number of clients not coherent with investigated setting. (3) Datasets not comparable. (4) Privacy: Usually identity protection OR gradient masking, not both.
%\end{enumerate}




%\subsection{Future Research Direction} \label{subsec:future_research_direction}

%\begin{enumerate}
   % \item KT: Application domains outside IoT/IoV e.g., FL for biomedical. ... in every domain where data is kept separately but the data holders would benefit of joint ML model training.
   % \item KT: Incentive mechanism using behavioral economics.
   % \item Privacy: overcome DP's problem of security-accuracy tradeoff, and/or MPC's problem of high computational effort.
%\end{enumerate}







==> table_FL.tex <==
\rowcolors{2}{tableoddrow}{tableevenrow}
% The command \rowcolors takes three parameters each passed inside braces:
% 1) the row to start,
% 2) the colour for odd rows and
% 3) the colour for even rows.
\begin{tabular}{C|CLCLL} 
    \rowcolor{tableheader} 
    Ref. & Application & Key Contribution & FL Setting & Actors & Setup period \\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LW %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \cite{LW1_witt2021rewardbased} & Generic & 1-bit Compressed Federated
Distillation on Blockchain with knowledge-free reward & n.s. &  Workers & \checkmark \\ 
    \cite{LW2_Weng2021} & Generic & Auditable and Decentralized Deep Learning with Blockchain-based secure and fair Incentive &n.s. &Workers & \checkmark \\
    \cite{LW3_Kumar2020} & Generic & Secure and decentralized FL against catastrophic forgetting & n.s. & Contributors, miners & \checkmark \\
    \cite{LW4_FL_IIoT} & IoT & Blockchain-Based Federated Learning for Device Failure Detection in IIoT & n.s. &  Clients, central organization & n.a. \\
    \cite{LW5_FL_HomeAppliances_IoT} & IoT & Privacy-preserving Blockchain-based FL system for smart home IoT & n.s. &  Clients, Miners &  \checkmark Manufacturer \\
    \cite{LW6_Rahmadika2020} & Generic & Incentivized Collaborative Learning Framework on Ethereum & n.s. & Agg. server and workers & \checkmark \\
    \cite{LW7_Zhang_Reputation} & Generic & Novel worker selection scheme based on reputation scores & n.s. & Worker, task publisher, miner & \xmark \\
    \cite{LW8_Privacy_IoV} & IoV & Improved DGHV encryption algorithm to solve the privacy problem for semi-honest and malicious MECs. & n.s. & MEC, macro base station (MBS), ADV & \xmark \\
    \cite{LW9_FedCoin} & Generic & Peer-to-Peer payment system for FL with proof of Shapley consensus blockchain & n.s. & Model requester, FL server, clients & \xmark \\
    \cite{LW10_refiner} & Generic & Incentive-driven FL system powered by blockchain & CD & Administrator, requester, worker, validator & \checkmark (Admin) \\
    \cite{LW11_RewardResponseGame} & Generic & Reward response game in the blockchain-powered FL system & n.s. & Central server, workers & \xmark \\
    \cite{LW12_Rahmadika2021_unlinkable} & Generic & Unlinkable collaborative learning transactions: privacy-awareness in decentralized approaches & CS & Workers, leaders, aggregation server & \xmark \\
    \cite{LW13_TowardsReputationINFOCOMM} & Generic & Blockchain-based reputation-aware and fine-grained federated learning & n.s. & Edge device, fog node, cloud & \checkmark \\
    \cite{LW14_5G_Rahmadika2021} & Generic & Blockchain-enabled cross-silo federated learning for 5G edge networks & CS & User, edge, cloud & \xmark  \\
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MH %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \cite{MH1_Chai2021}beginMH & IoV &  Hierachical FL framework with two-layered blockchain embedded for scalability & CD & Vehicles, roadside units, base stations & \xmark \\
    \cite{MH2_Kang2019} & Generic &  Reputation-based incentive mechanism for FL & CD & Task publisher, workers & \xmark \\
    \cite{Bao2019FLChain} & Generic &  FL framework with custom federation establishment algorithm for ideal profit distribution & n.s. & Participant/trainer, buyer, reporter, data processor & \checkmark \\
    \cite{MH4_Ma2021} & Generic &  Secure contribution measurement through group-based Shapley value computation for horizontal FL & CS & Data owner & \checkmark \\
    \cite{MH5_Lei2021} & IoT &  Two-layered blockchain architecture for scalable FL & CD & Local devices, base stations, mobile edge computing nodes & \checkmark \\
    \cite{MH6_Kansra2022} & IoV &  Integration of data augmentation into FL incentive design & CD & Vehicle edge nodes, BC nodes & \xmark \\
    \cite{MH7_Mugunthan2022} & Generic & FL framework with custom contribution scoring procedure & n.s.& Trainer nodes & \checkmark \\
    \cite{MH8_Fadaeddini2019} & Generic &  Blockchain enabled FL framework with adaptive participation cost & n.s. & Model initiator, computing partner, validator & \xmark \\
    \cite{MH9_He2021} & Finance &  Framework for horizontal and vertical FL with custom contribution measurement and incentive design & CS & Follower candidate, leader nodes & \checkmark \\
    \cite{MH10_Qu2021} & IoT & FL framework for offloading decision making with custom consensus mechanism & CD & Users, edge server, cloud server &  \xmark\\
    \cite{MH11_Desai2021} & Generic & Prevention of backdoor attacks through hybrid blockchain enables accountability & CD & Worker nodes & \checkmark \\
    \cite{MH12_Zhu2021} & Generic & Privacy-preserving decentralized federated deep learning framework  & n.s. & Task publisher, parties, miners, smart contract & \checkmark \\
    \cite{MH13_Li2020} & Generic &  Elgamal enabled secure FL framework with custom scoring evaluation mechanism and  & n.s. & Requesters, workers, crowdsourcing platform & \xmark \\
    \cite{MH14_Rathore2019}endMH & IoT & FL framework with reduced blockchain induced latency and computational overhead & n.s. & IoT device, edge server, central cloud server & \xmark \\
    
    
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \cite{KT01_Toyoda2019BigData, KT02_Toyoda2020Access} & Generic & Reward distribution based on votes & n.s. & Requesters and workers & \checkmark \\
   \cite{KT03_Martinez2019CyberC} & Generic & Validation error based metric for contribution measurement & n.s. & Requesters, workers	& \xmark \\
    \cite{KT04_Zou2021WCNC} & IoV & Regional FL for IoV & CD & Road side units (RSUs) as aggregators, MECs, vehicles (workers) & \xmark \\
    \cite{KT05_Hu2021IoTJ} & IoT & Privacy-preserving crowdsensing with FL and MD & n.s. & Requesters, workers (edge servers), data collectors & \xmark \\
    \cite{KT06_Wang2021TNSE} & IoV (UAV) & Privacy-preserving FL for UAV with two-tier reinforcement learning & n.s. & UAVs (sensors, workers), requesters, MECs & \xmark \\
    \cite{KT07_Ur_Rehman2020INFOCOMW} & Generic & Three-tier fine-grained FL architecture (on device, edge and cloud) wth reputation & n.s & Requesters (cloud servers), data-arbitrators (fog nodes), workers (edge-devices) & \xmark \\
    \cite{KT08_Qu2021TPDS} & Generic & A consensus algorithm that replaces PoW with FL & n.s. & Requesters, miners & \xmark \\
    \cite{KT09_Zhang2021IJHPSA} & Generic & A consensus algorithm that replaces double hashing adopted to a traditional PoW with Huffman coding & n.s. & Miners, workers & \xmark \\
    \cite{KT10_Gao2021ICPP} & Generic & Fair reward distribution with contribution measurement and reputation & n.s. & Requesters, workers, aggregation servers & \xmark \\
    \cite{KT11_Xuan2021SCN} & Generic & Reducing communications cost of \cite{KT01_Toyoda2019BigData} & n.s. & Administrator, requesters, workers, miners & \xmark \\
    \cite{KT12_Liu2021Sensors} & Generic & Aggregation by randomly selected miners to avoid single point of failure & CS and CD & Workers, miners & \xmark \\
   
\end{tabular}
